REACT to Cyber Attacks on Power Grids

Motivated by the recent cyber attack on the Ukrainian power grid, we study cyber attacks on power grids that affect both the physical infrastructure and the data at the control center. In particular, we assume that an adversary attacks an area by: (i) remotely disconnecting some lines within the attacked area, and (ii) modifying the information received from the attacked area to mask the line failures and hide the attacked area from the control center. For the latter, we consider two types of attacks: (i) data distortion: which distorts the data by adding powerful noise to the actual data, and (ii) data replay: which replays a locally consistent old data instead of the actual data. We use the DC power flow model and prove that the problem of finding the set of line failures given the phase angles of the nodes outside of the attacked area is strongly NP-hard, even when the attacked area is known. However, we introduce the polynomial time REcurrent Attack Containment and deTection (REACT) Algorithm to approximately detect the attacked area and line failures after a cyber attack. We numerically show that it performs very well in detecting the attacked area, and detecting single, double, and triple line failures in small and large attacked areas.

==> Sources/Building_Blocks.tex <==
\section{Detection and Correction}\label{sec:buidlingblocks}
In this section, we provide the building blocks of the REACT Algorithm to detect the attacked area $H$ and line failures $F$.
\subsection{Attacked Area Containment}\label{subsec:contain}

Since $\tet_H^{\star}$ is the vector of the modified phase angles and there are also some line failures in $H$, it can be seen that $\A\tet^{\star}\neq \vec{p}$.
\begin{lemma}\label{lem:Hbar_int}
For any $i\in \intt(\bar{H})$, $\A_i\tet^{\star}=p_i$.
\end{lemma}
\begin{proof}
Since $i\in \intt(\bar{H})$, therefore $a_{ij}=0$ for all $j\in V_H$. Hence, $\A_i\tet^{\star}=\A_{i|\bar{H}}\tet_{\bar{H}}^{\star}$. On the other hand, since the attack is inside $H$, we know $\A_{i|\bar{H}}=\A_{i|\bar{H}}'$, and also $\tet_{\bar{H}}^{\star}=\tet_{\bar{H}}'$. Hence, $\A_i\tet^{\star}=\A_{i|\bar{H}}\tet_{\bar{H}}^{\star}=\A_{i|\bar{H}}'\tet_{\bar{H}}'=p_i$.
\end{proof}
\begin{lemma}\label{lem:not_int}
For any $i\in V\backslash \intt(\bar{H})$, $\A_i\tet^{\star}\neq p_i$ almost surely.
\end{lemma}
\begin{proof}
For any $i\in V\backslash\intt(\bar{H})$, there exists a node $j\in V_H$ such that $a_{ij}\neq 0$. Now since the set of solutions $\vec{x}$ to $\A_i\vec{x}= p_i$ is a measure zero set in $\mathbb{R}^n$ and $\theta_j^{\star}$ is a random modification of $\theta_j'$, $\A_i\tet^{\star}\neq p_i$ almost surely.
\end{proof}
Lemmas~\ref{lem:Hbar_int} and \ref{lem:not_int} indicate that given $\A,\tet,$ and $\tet^{\star}$ one can find $\intt(\bar{H})$ by computing $V\backslash \supp(\A\tet^{\star}- \vec{p})$.
\begin{corollary}\label{cor:int_Hbar}
$\intt(\bar{H})=V\backslash \supp(\A\tet^{\star}- \vec{p})$, almost surely.
\end{corollary}

Following Corollary~\ref{cor:int_Hbar}, one can contain the attacked area as depicted in Fig.~\ref{fig:attack_containment}. The green nodes show the $\intt(\bar{H})$ and yellow nodes show $\supp(\A\tet^{\star}- \vec{p})$. We refer to the nodes in $\supp(\A\tet^{\star}- \vec{p})$ as \emph{suspicious nodes} and denote the subgraph induced by the suspicious nodes by $S_1$.
\subsection{Attacked Area Approximation}\label{subsec:approx}
\begin{figure}[t]
\centering
\includegraphics[scale=0.35]{Figures/Attack_model_118_sus_nodes_levels_border.png}
\vspace*{-0.2cm}
\caption{$H$ is an induced subgraph of $G$ that represents the  attacked area. The red, orange, and yellow nodes represent the nodes in $S_3$, $S_2\backslash S_3$, and $S_1\backslash S_2$, respectively.}
%Thus, after the attack the phase angles of the nodes and the status of the lines in $H$ become unavailable to the control center.}
\label{fig:attack_containment}
%\vspace*{-0.5cm}
\end{figure}
Given the set of suspicious nodes $V_{S_1}$, we know from corollary~\ref{lem:Hbar_int} that $\intt(\bar{H})=V_{\bar{S}_1}$ and from Lemma~\ref{lem:not_int} that $V_H\subset V_S$. Therefore, $S_1$ can approximate $H$. In this subsection, we want to improve our approximation by removing some nodes from $S_1$.  To do so, we first in the following lemma show that $\intt(S_1)$ is a better approximation for $V_H$.
\begin{lemma}\label{lem:estimate_H1}
$V_H\subseteq \intt(S_1)$, almost surely.
\end{lemma}
\begin{proof}
Assume not, there should exists a node $i\in V_H$ such that $N(i)\cap V_{\bar{S}_1}\neq \emptyset$. Assume $j\in N(i)\cap V_{\bar{S}_1}\neq \emptyset$, then with a similar argument as in the proof of Lemma~\ref{lem:not_int}, one can show that $\A_j\tet^{\star}\neq p_j$ almost surely, which contradicts with $j\in V_{\bar{S}_1}$ following Lemma~\ref{lem:Hbar_int}. Hence, $N(i)\cap V_{\bar{S}_1} = \emptyset$ and $V_H\subseteq \intt(S_1)$.
\end{proof}
Following Lemma~\ref{lem:estimate_H1}, $S_2:=G[\intt(S_1)]$ is a better approximation for the attacked area $H$.  In order to find a more accurate approximation for $H$, we provide the following lemma which is similar to \cite[Lemma 1]{SYZ2015}.
\begin{lemma}\label{lem:StoH}
For a subgraph $S$, if $V_H\subseteq V_S$, then:
\begin{equation}\label{eq:StoH}
\A_{\bar{S}|G} (\tet-\tet') = 0.
\end{equation}
\end{lemma}
\begin{proof}
Since all the line failures are inside $H$, and also $V_H\subseteq V_S$, therefore it can be seen that $\A_{\bar{S}|G} = \A_{\bar{S}|G}'$. On the other hand, $\A_{\bar{S}|G}\tet = \vec{p}_{\bar{S}}$ and $\A_{\bar{S}|G}'\tet' = \vec{p}_{\bar{S}}$. Hence, $\A_{\bar{S}|G}\tet - \A_{\bar{S}|G}'\tet'=0$ and therefore $\A_{\bar{S}|G} (\tet-\tet') = 0$.
\end{proof}

Lemma~\ref{lem:StoH} can be effectively used to estimate the phase angle of the nodes in $S$ and to detect the attacked area $H$ using these estimate values. The idea is to break (\ref{eq:StoH}) into parts that are known and unknown as follows:
\begin{align*}
\A_{\bar{S}|\bar{S}} (\tet_{\bar{S}}-\tet'_{\bar{S}}) + \A_{\bar{S}|S} (\tet_{S}-\tet'_{S}).
\end{align*}
Notice that since $V_H\subseteq V_S$, therefore $\tet'_{\bar{S}}=\tet^{\star}_{\bar{S}}$. Hence, the only unknown variable in equation above is $\tet'_{S}$. Assume $\vec{y}\in \mathbb{R}^{|V_S|}$ is a solution to the following equation:
\begin{equation}\label{eq:H_detect}
\A_{\bar{S}|S} \vec{y} = \A_{\bar{S}|\bar{S}} (\tet_{\bar{S}}-\tet^{\star}_{\bar{S}}) + \A_{\bar{S}|S} \tet_{S},
\end{equation}
in the following lemma, we demonstrate that $\supp(\vec{y}-\tet^{\star}_{S})$ can be used to estimate $H$.
\begin{lemma}\label{lem:estimate_H2}
If $\vec{y}$ is a solution to (\ref{eq:H_detect}), $V_H\subseteq \supp(\vec{y}-\tet^{\star}_{S})$.
\end{lemma}
Following Lemma~\ref{lem:estimate_H2}, if $\vec{y}$ is a solution to (\ref{eq:H_detect}) for $S=S_2$, then $S_3:=G[\supp(\vec{y}-\tet^{\star}_{S_2})]$ would be a better approximation for the attacked area $H$. Fig.~\ref{fig:attack_containment} shows the difference between $S_1$, $S_2$, and $S_3$ in approximating the attacked area.

Finally, the following lemma demonstrate when $S_3$ is an exact approximation of $H$.
\begin{lemma}\label{lem:exact}
For a subgraph $S$ such that $V_H\subseteq V_S$, if $V_S\backslash V_H\subseteq \partial(S)$ and there is a matching between the nodes in $\bar{S}$ and $\partial(S)$ that covers all the nodes in $\partial(S)$, then $G[\supp(\vec{y}-\tet^{\star}_{S})]=H$, in which $\vec{y}$ is the solution to (\ref{eq:H_detect}).
\end{lemma}
\begin{proof}
\end{proof}
\subsection{Line Failures Detection}\label{subsec:detect}
In the previous subsection, we demonstrated that $S_3$ provides a good approximation for the attacked area $H$. In this section, we provide a method to detect line failures inside $S = S_3$. For this reason,  we use and build on the idea introduced in~\cite{SYZ2015}. It was proved in~\cite{SYZ2015} that if the attacked area $H$ is known, then there exist vectors $\vec{x}\in\mathbb{R}^{|E_H|}$ and $\vec{y}\in\mathbb{R}^{|V_H|}$ satisfying following optimization problem such that $\supp(\vec{x})=F$ and $\vec{y}=\tet_H'$:
\begin{eqnarray}\label{eq:simul_detect}
&&\min_{\vec{x},\vec{y}} \|\vec{x}\|_1~\text{s.t.}\nonumber\\
&&\A_{H|H}(\tet_H-\vec{y})+\A_{H|\bar{H}}(\tet_{\bar{H}}-\tet'_{\bar{H}})=\D_H\vec{x}\\
&&\A_{\bar{H}|H}(\tet_H-\vec{y})+\A_{\bar{H}|\bar{H}}(\tet_{\bar{H}}-\tet'_{\bar{H}})=0.\nonumber
\end{eqnarray}

The novelty of this method is that it provides a convex relaxation for the line failures detection problem which is combinatorial in nature (as we showed in Section~\ref{sec:hardness}).
Notice that  the  optimization problem~(\ref{eq:simul_detect}) can be solved efficiently using Linear Program (LP). It is proved that under some conditions on $H$ and the set of line failures $F$, the solution to~(\ref{eq:simul_detect}) is unique, therefore the relaxation is exact and the set of line failures can be detected by solving~(\ref{eq:simul_detect}). In particular, it is proved in~\cite{SYZ2015} that if $H$ is acyclic and there is a matching between the nodes in $H$ and $\bar{H}$ that covers $H$, the solution to~(\ref{eq:simul_detect}) is unique for any set of line failures.

Since the conditions on $H$ and $F$ as described in~\cite{SYZ2015} may not always hold for the exactness of the line failures detection using (\ref{eq:simul_detect}), therefore it cannot be used in general cases to detect line failures. To address this issue, here, we introduce a randomized version of the optimization problem (\ref{eq:simul_detect}).


Assume $\W \in \mathbb{R}^{|E_S|\times |E_S|}$ is a diagonal matrix, we show that the solution to the following optimization problem can detect line failures in $S$ accurately for a ``good" weight matrix $\W$:
\begin{eqnarray}\label{eq:weighted_simul_detect}
&&\min_{\vec{x},\vec{y}} \|\W\vec{x}\|_1~\text{s.t.}\nonumber\\
&&\A_{S|S}(\tet_S-\vec{y})+\A_{S|\bar{S}}(\tet_{\bar{S}}-\tet'_{\bar{S}})=\D_S\vec{x}\\
&&\A_{\bar{S}|S}(\tet_S-\vec{y})+\A_{\bar{S}|\bar{S}}(\tet_{\bar{S}}-\tet'_{\bar{S}})=0.\nonumber
\end{eqnarray}
%\subsection{Confidence Computation}
The idea behind optimizing the weighted norm-1 of vector $\vec{x}$ is to be able to detect the line failures when the solution to (\ref{eq:simul_detect}) does not detect the correct set of line failures but a small disturbance results in the correct detection.

Before we demonstrate the effectiveness of the optimization (\ref{eq:weighted_simul_detect}) in detecting line failures, we provide a metric for measuring the \emph{confidence of a solution} and use that to define delectability of a set of line failures. In a subgraph $S$ such that $V_H\subseteq V_S$, assume $F^{\dagger}$ and $\pvec{\theta}_S^{\dagger}$ are the set of detected line failures and the recovered phase angles, respectively. Also assume that $\A^{\dagger}$ is the admittance matrix after removing the lines in $F^{\dagger}$ and define $\pvec{p}^{\dagger}:=\A_{G|\bar{S}}\tet'_{\bar{S}}+\A_{G|S}^{\dagger}\pvec{\theta}^{\dagger}_S$.
\begin{definition}
 The \emph{confidence of the solution} is denoted by $c(F^{\dagger},\pvec{\theta}_S^{\dagger})$ and defined as:
\begin{equation}\label{eq:confidence}
c(F^{\dagger},\pvec{\theta}_S^{\dagger}) := (1-\|\pvec{p}^{\dagger} - \vec{p}\|_2/\|\vec{p}\|_2)^+\times100,
\end{equation}
in which $(x)^+ := \max(0,x)$.
\end{definition}

\begin{definition}\label{eq:detectable}
The set of line failures in $H$ is called \emph{detectable} if there exist a unique set $F^{\dagger}\subseteq E_H$ and a vector $\pvec{\theta}^{\dagger}_H$ such that $c(F^{\dagger},\pvec{\theta}_H^{\dagger})=100\%$.
\end{definition}

The confidence of the solution along with a random selection of the weight matrix $\W$ in (\ref{eq:weighted_simul_detect}) can be used to detect line failures that cannot be detected using (\ref{eq:simul_detect}). The idea is to repeatedly solve (\ref{eq:weighted_simul_detect}) using random weight matrix  until the confidence of the solution for $F^{\dagger}=\supp(\vec{x})$ and $\pvec{\theta}_S^{\dagger}=\vec{y}$ is 100\%. In the rest of this section, we demonstrate why this approach is effective and when the expected number of repetitions is polynomial in terms of the input size. Here, We consider the case when the diagonal entries of matrix $\W$ are drown randomly from an exponential distribution. %The following two lemmas demonstrate how (\ref{eq:weighted_simul_detect}) can result in the correct detection when (\ref{eq:simul_detect}) does not.

\begin{lemma}\label{lem:expdistbound}
Assume $w_1,w_2,\dots,w_m$ are i.i.d.\ exponential random variables with rate $\lambda$, then for $1\leq k\leq m-1$:
\begin{equation*}
Pr(\sum_{i=1}^k w_i<\sum_{i=k+1}^m w_i)= 1-\frac{\sum_{j=0}^{k-1}\binom{m-1}{j}}{2^{m-1}}.
\end{equation*}
\end{lemma}
\begin{corollary}\label{cor:expdistbound}
Assume $w_1,w_2,\dots,w_m$ are i.i.d.\ exponential random variables with rate $\lambda$, then for $k = m/2+\Theta(\sqrt{m})$:
\begin{equation*}
Pr(\sum_{i=1}^k w_i<\sum_{i=k+1}^m w_i)= \frac{1}{2^{O(1/m)}\Theta(\sqrt{m})}.
\end{equation*}
\end{corollary}

%\begin{corollary}\label{cor:expdistbound}
%Assume $w_1,w_2,\dots,w_m$ are i.i.d.\ exponential random variables with rate $\lambda$, then for $1\leq k\leq \lfloor (m-1)/2\rfloor$:
%\begin{equation*}
%Pr(\sum_{i=1}^k w_i<\sum_{i=k+1}^m w_i)\geq \frac{1}{2},
%\end{equation*}
%and for $\lfloor (m-1)/2\rfloor<k\leq \lfloor (m-1)/2\rfloor+\sqrt{m-1}/2$:
%\begin{equation*}
%Pr(\sum_{i=1}^k w_i<\sum_{i=k+1}^m w_i)= \Theta(1),
%\end{equation*}
%\end{corollary}

\begin{lemma}\label{lem:cycle}
If $S=H$, $H$ is a cycle, and there is a matching between the nodes inside and outside of $H$ that covers all the inside nodes, then any set of line failures of size $k$ can be found by solving (\ref{eq:weighted_simul_detect}) expectedly $2^{m-1}/(2^{m-1}-\sum_{j=0}^{k-1}\binom{m-1}{j})$ times for random matrices $\W$.
\end{lemma}

Lemma~\ref{lem:cycle} clearly demonstrates the effectiveness of using a weight matrix $\W$ in (\ref{eq:weighted_simul_detect}). It was previously proved in~\cite{SYZ2015} that if $H$ is a cycle and there is a matching between the nodes inside and outside of $H$ that covers all the inside nodes, then for any set of line failures of size \emph{less than half of the lines in $H$}, $\supp(\vec{x})$ of the solution $\vec{x}$ to (\ref{eq:simul_detect}) exactly reveals the set of line failures. However, for the line failures with the size more than half of the lines in $H$, this approach comes short. In these cases, Lemma~\ref{lem:cycle} indicates that solving (\ref{eq:weighted_simul_detect}) for random matrices $\W$ for polynomial number of times can lead to the correct detection. 

\begin{lemma}\label{lem:star}
If $S=H$, $H$ is a star, and there is a matching between the nodes inside and outside of $H$ that covers all the inside nodes except the central node of the star, then any set of line failures of size $k$ can be found by solving (\ref{eq:weighted_simul_detect}) expectedly $2^{m-1}/(2^{m-1}-\sum_{j=0}^{k-1}\binom{m-1}{j})$ times for random matrices $\W$.
\end{lemma}
%In the following lemma, we demonstrate that for any attacked area $H$ and a detectable set of line failures $F$, there exist a weight matrix $\W$ such that the solution to (\ref{eq:weighted_simul_detect}) reveals the set of line failures correctly.
%\begin{lemma}\label{lem:W}
%If the set of line failures in $H$ are detectable and $S=H$, then there exists a diagonal matrix $\W\in\mathbb{R}^{|E_S|\times |E_S|}$ such that the solution $\vec{x},\vec{y}$ to (\ref{eq:weighted_simul_detect}) is unique, $\supp(\vec{x})=F$, and $\vec{y}=\tet'_H$.
%\end{lemma} 
